On Reconfigurability of Target Sets

We study the problem of deciding reconfigurability of target sets of a graph. Given a graph $G$ with vertex thresholds $\tau$, consider a dynamic process in which vertex $v$ becomes activated once at least $\tau(v)$ of its neighbors are activated. A vertex set $S$ is called a target set if all vertices of $G$ would be activated when initially activating vertices of $S$. In the Target Set Reconfiguration problem, given two target sets $X$ and $Y$ of the same size, we are required to determine whether $X$ can be transformed into $Y$ by repeatedly swapping one vertex in the current set with another vertex not in the current set preserving every intermediate set as a target set. In this paper, we investigate the complexity of Target Set Reconfiguration in restricted cases. On the hardness side, we prove that Target Set Reconfiguration is PSPACE-complete on bipartite planar graphs of degree $3$ and $4$ and of threshold $2$, bipartite $3$-regular graphs and planar $3$-regular graphs of threshold $1$ and $2$, and split graphs, which is in contrast to the fact that a special case called Vertex Cover Reconfiguration is in P for the last graph class. On the positive side, we present a polynomial-time algorithm for Target Set Reconfiguration on graphs of maximum degree $2$ and trees. The latter result can be thought of as a generalization of that for Vertex Cover Reconfiguration.

==> fig_cycle-odd-temp.tex <==
\coordinate(w1) at ({3*cos(5*pi/10 r)},{3*sin(5*pi/10 r)});
\coordinate(w2) at ({3*cos(1*pi/10 r)},{3*sin(1*pi/10 r)});
\coordinate(w3) at ({3*cos(-3*pi/10 r)},{3*sin(-3*pi/10 r)});
\coordinate(w4) at ({3*cos(-7*pi/10 r)},{3*sin(-7*pi/10 r)});
\coordinate(w5) at ({3*cos(-11*pi/10 r)},{3*sin(-11*pi/10 r)});
\coordinate(a) at ($(w1)!0.50!(w2)$);
\coordinate(b) at ($(w2)!0.30!(w3)$);
\coordinate(c) at ($(w2)!0.50!(w3)$);
\coordinate(d) at ($(w3)!0.25!(w4)$);
\coordinate(e) at ($(w3)!0.45!(w4)$);
\coordinate(f) at ($(w3)!0.65!(w4)$);
\coordinate(g) at ($(w4)!0.50!(w5)$);
\coordinate(h) at ($(w5)!0.30!(w1)$);
\coordinate(i) at ($(w5)!0.50!(w1)$);

\foreach \u/\v in {w1/w2, w2/w3, w3/w4, w4/w5, w5/w1}
    \draw[myedge] (\u)--(\v);

\draw(w1) node[mynode]{$w_1$};
\draw(w2) node[mynode]{$w_2$};
\draw(w3) node[mynode]{$w_3$};
\draw(w4) node[mynode]{$w_4$};
\draw(w5) node[mynode]{$w_5$};
\foreach \v in {a,b,c,d,e,f,g,h,i}
    \draw(\v) node[mymynode]{};

%        \foreach \u/\v in {w1/a, w2/c, w3/f, w4/g, w5/i}
%            \draw[densely dashed, thick] \convexpath{\u,\v}{5.5mm};
\node[mylabel, font=\LARGE, left=6mm of w1]  {$I_1$};
\node[mylabel, font=\LARGE, right=6mm of w2] {$I_2$};
\node[mylabel, font=\LARGE, right=6mm of w3] {$I_3$};
\node[mylabel, font=\LARGE, left=6mm of w4]  {$I_4$};
\node[mylabel, font=\LARGE, left=6mm of w5]  {$I_5$};


==> fig_tree-lem.tex <==
\begin{figure}[tbp]
    \centering
    \scalebox{0.7}{\begin{tikzpicture}
        \input{fig_tree-temp1}
        \path[pattern=north east lines] \convexpath{r,h,m,i,e}{6mm};
        \draw[draw=none, fill=white] \convexpath{a,d,f,c}{6mm};
        \draw[densely dashed, thick] \convexpath{a,d,b}{6mm};
        \input{fig_tree-temp2}
        \node at (1.8,-1.8) {\LARGE $Q_4$};
        \node[inner sep=0.5mm, fill=white] at (-1,-5.5) {\LARGE $S_4$};
    \end{tikzpicture}}
    \caption{
        The proof of \cref{lem:tree-chara}.
        Each vertex $v$ is associated with a pair of $\tau(v)$ and $\tau'(v)$, denoted $\tau(v) : \tau'(v)$.
        $S_4 = V(G) \setminus P_4$ is denoted by diagonal lines;
        $Q_4$ is denoted by a dashed line.
        $S'_4$ is defined as $S_4 \uplus \{v_0\}$, which turn out not to be a target set.
    }
    \label{fig:tree-lem}
\end{figure}

